Health Text Simplification: An Annotated Corpus for Digestive Cancer Education and Novel Strategies for Reinforcement Learning

Objective: The reading level of health educational materials significantly influences the understandability and accessibility of the information, particularly for minoritized populations. Many patient educational resources surpass the reading level and complexity of widely accepted standards. There is a critical need for high-performing text simplification models in health information to enhance dissemination and literacy. This need is particularly acute in cancer education, where effective prevention and screening education can substantially reduce morbidity and mortality. Methods: We introduce Simplified Digestive Cancer (SimpleDC), a parallel corpus of cancer education materials tailored for health text simplification research, comprising educational content from the American Cancer Society, Centers for Disease Control and Prevention, and National Cancer Institute. Utilizing SimpleDC alongside the existing Med-EASi corpus, we explore Large Language Model (LLM)-based simplification methods, including fine-tuning, reinforcement learning (RL), reinforcement learning with human feedback (RLHF), domain adaptation, and prompt-based approaches. Our experimentation encompasses Llama 2 and GPT-4. A novel RLHF reward function is introduced, featuring a lightweight model adept at distinguishing between original and simplified texts, thereby enhancing the model's effectiveness with unlabeled data. Results: Fine-tuned Llama 2 models demonstrated high performance across various metrics. Our innovative RLHF reward function surpassed existing RL text simplification reward functions in effectiveness. The results underscore that RL/RLHF can augment fine-tuning, facilitating model training on unlabeled text and improving performance.

==> diff_sections/data.tex <==


\DIFaddbegin \DIFadd{We provide the new SimpleDC corpus to the research community to advance health text simplification.}\footnote{\href{https://github.com/mushfiqur11/simpledc-dataset.git}{\DIFadd{https://github.com/mushfiqur11/simpledc-dataset.git}}} \DIFadd{In developing SimpleDC, we utilized publicly available text data from the NCI, ACS, and CDC websites with the goal of advancing text simplification and public health communication. Our use of this data is in alignment with fair use principles, as the data was employed exclusively for academic and research purposes, without any commercial intent. We minimized data usage, extracting only the portions necessary to support our work on text simplification and public health communication. Furthermore, our use of the data does not adversely affect the market value or potential of the original content. The text data from the NCI, ACS, and CDC was specifically used to improve NLP methods that enhance the accessibility of health information, with all sources carefully attributed. SimpleDC is made publicly available, with detailed source attribution, ensuring full transparency and traceability. }\DIFaddend

==> tables/domain_adaptation.tex <==
\begin{table}[ht!]
\small
\centering
\begin{tabular}{l|l|cccccc}
\toprule
\textbf{Model Name}                                                      & \textbf{RLHF Reward}  & \multicolumn{1}{l}{\textbf{SARI}} & \multicolumn{1}{l}{\textbf{BLEU}} & \multicolumn{1}{l}{\textbf{BERTScore}} & \multicolumn{1}{l}{\textbf{ROUGE}} & \multicolumn{1}{l}{\textbf{FKGL}} \\ \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Llama-2-7b-\\ chat-hf\end{tabular}}      & none                    & 35.15 & 0.52 & 0.94 & 0.64 & 8.49 \\ 
& $R_{FKGL}+R_{Rel}$      & 45.71 & 0.63 & 0.96 & 0.78 & 7.50 \\ 
& $R_{FKGL}+R_{OvS}$      & 74.41 & 0.73 & 0.97 & 0.89 & 7.74 \\ 
\midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Llama-2-7B-\\ 32K-Instruct\end{tabular}} & none                    & 26.70 & 0.36 & 0.92 & 0.52 & 8.25 \\ 
& $R_{FKGL}+R_{Rel}$      & 37.55 & 0.58 & 0.95 & 0.72 & 7.45 \\ 
& $R_{FKGL}+R_{OvS}$      & 45.71 & 0.63 & 0.96 & 0.78 & 7.50 \\
\bottomrule
\end{tabular}
\caption{Results of domain adaptation experimentation on SimpleDC dataset}
\label{domain_adaptation}
\end{table}
